Statistical Mechanics of a Thin Film on a Solid Substrate

We study the behavior of very thin liquid films wetting homogeneous planar and spherical substrates. In order to describe a simple fluid at very small scales, we employ a classical density functional theory (DFT). Here, we model a fluid with a local density approximation (LDA) for its hard-sphere contribution and assume that the intermolecular attractive forces are long-range. In particular, we first introduce the basic concept of DFT, and then present computations for fluid films on planar and spherically symmetric walls. We present equilibrium density profiles and adsorption isotherms. We also compare our results to predictions from a sharp-interface approximation (SIA) and suggest a piecewise function approximation (PFA), which assumes that the density profile at the wall-liquid and the liquid-vapor interfaces varies smoothly.

==> Mu_Over_T.tex <==
% GNUPLOT: LaTeX picture
\setlength{\unitlength}{0.240900pt}
\ifx\plotpoint\undefined\newsavebox{\plotpoint}\fi
\begin{picture}(1500,900)(0,0)
\sbox{\plotpoint}{\rule[-0.200pt]{0.400pt}{0.400pt}}%
\put(466.0,131.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(446,131){\makebox(0,0)[r]{-5.2}}
\put(1175.0,131.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(466.0,204.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(446,204){\makebox(0,0)[r]{-5}}
\put(1175.0,204.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(466.0,277.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(446,277){\makebox(0,0)[r]{-4.8}}
\put(1175.0,277.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(466.0,350.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(446,350){\makebox(0,0)[r]{-4.6}}
\put(1175.0,350.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(466.0,423.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(446,423){\makebox(0,0)[r]{-4.4}}
\put(1175.0,423.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(466.0,496.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(446,496){\makebox(0,0)[r]{-4.2}}
\put(1175.0,496.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(466.0,568.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(446,568){\makebox(0,0)[r]{-4}}
\put(1175.0,568.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(466.0,641.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(446,641){\makebox(0,0)[r]{-3.8}}
\put(1175.0,641.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(466.0,714.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(446,714){\makebox(0,0)[r]{-3.6}}
\put(1175.0,714.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(466.0,787.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(446,787){\makebox(0,0)[r]{-3.4}}
\put(1175.0,787.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(466.0,860.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(446,860){\makebox(0,0)[r]{-3.2}}
\put(1175.0,860.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(466.0,131.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(466,90){\makebox(0,0){ 0.2}}
\put(466.0,840.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(556.0,131.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(556,90){\makebox(0,0){ 0.3}}
\put(556.0,840.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(646.0,131.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(646,90){\makebox(0,0){ 0.4}}
\put(646.0,840.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(736.0,131.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(736,90){\makebox(0,0){ 0.5}}
\put(736.0,840.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(826.0,131.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(826,90){\makebox(0,0){ 0.6}}
\put(826.0,840.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(916.0,131.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(916,90){\makebox(0,0){ 0.7}}
\put(916.0,840.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(1006.0,131.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(1006,90){\makebox(0,0){ 0.8}}
\put(1006.0,840.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(1096.0,131.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(1096,90){\makebox(0,0){ 0.9}}
\put(1096.0,840.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(1186.0,131.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(1186,90){\makebox(0,0){ 1}}
\put(1186.0,840.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(466.0,131.0){\rule[-0.200pt]{0.400pt}{175.616pt}}
\put(466.0,131.0){\rule[-0.200pt]{175.616pt}{0.400pt}}
\put(1195.0,131.0){\rule[-0.200pt]{0.400pt}{175.616pt}}
\put(466.0,860.0){\rule[-0.200pt]{175.616pt}{0.400pt}}
\put(325,495){\makebox(0,0){$\mu$}}
\put(830,29){\makebox(0,0){T}}
\put(466,178){\usebox{\plotpoint}}
\multiput(466.58,178.00)(0.494,1.523){27}{\rule{0.119pt}{1.300pt}}
\multiput(465.17,178.00)(15.000,42.302){2}{\rule{0.400pt}{0.650pt}}
\multiput(481.58,223.00)(0.494,1.421){27}{\rule{0.119pt}{1.220pt}}
\multiput(480.17,223.00)(15.000,39.468){2}{\rule{0.400pt}{0.610pt}}
\multiput(496.58,265.00)(0.494,1.452){25}{\rule{0.119pt}{1.243pt}}
\multiput(495.17,265.00)(14.000,37.420){2}{\rule{0.400pt}{0.621pt}}
\multiput(510.58,305.00)(0.494,1.215){27}{\rule{0.119pt}{1.060pt}}
\multiput(509.17,305.00)(15.000,33.800){2}{\rule{0.400pt}{0.530pt}}
\multiput(525.58,341.00)(0.494,1.147){27}{\rule{0.119pt}{1.007pt}}
\multiput(524.17,341.00)(15.000,31.911){2}{\rule{0.400pt}{0.503pt}}
\multiput(540.58,375.00)(0.494,1.079){27}{\rule{0.119pt}{0.953pt}}
\multiput(539.17,375.00)(15.000,30.021){2}{\rule{0.400pt}{0.477pt}}
\multiput(555.58,407.00)(0.494,1.084){25}{\rule{0.119pt}{0.957pt}}
\multiput(554.17,407.00)(14.000,28.013){2}{\rule{0.400pt}{0.479pt}}
\multiput(569.58,437.00)(0.494,0.942){27}{\rule{0.119pt}{0.847pt}}
\multiput(568.17,437.00)(15.000,26.243){2}{\rule{0.400pt}{0.423pt}}
\multiput(584.58,465.00)(0.494,0.873){27}{\rule{0.119pt}{0.793pt}}
\multiput(583.17,465.00)(15.000,24.353){2}{\rule{0.400pt}{0.397pt}}
\multiput(599.58,491.00)(0.494,0.839){27}{\rule{0.119pt}{0.767pt}}
\multiput(598.17,491.00)(15.000,23.409){2}{\rule{0.400pt}{0.383pt}}
\multiput(614.58,516.00)(0.494,0.827){25}{\rule{0.119pt}{0.757pt}}
\multiput(613.17,516.00)(14.000,21.429){2}{\rule{0.400pt}{0.379pt}}
\multiput(628.58,539.00)(0.494,0.702){27}{\rule{0.119pt}{0.660pt}}
\multiput(627.17,539.00)(15.000,19.630){2}{\rule{0.400pt}{0.330pt}}
\multiput(643.58,560.00)(0.494,0.668){27}{\rule{0.119pt}{0.633pt}}
\multiput(642.17,560.00)(15.000,18.685){2}{\rule{0.400pt}{0.317pt}}
\multiput(658.58,580.00)(0.494,0.634){27}{\rule{0.119pt}{0.607pt}}
\multiput(657.17,580.00)(15.000,17.741){2}{\rule{0.400pt}{0.303pt}}
\multiput(673.58,599.00)(0.494,0.644){25}{\rule{0.119pt}{0.614pt}}
\multiput(672.17,599.00)(14.000,16.725){2}{\rule{0.400pt}{0.307pt}}
\multiput(687.58,617.00)(0.494,0.566){27}{\rule{0.119pt}{0.553pt}}
\multiput(686.17,617.00)(15.000,15.852){2}{\rule{0.400pt}{0.277pt}}
\multiput(702.00,634.58)(0.497,0.494){27}{\rule{0.500pt}{0.119pt}}
\multiput(702.00,633.17)(13.962,15.000){2}{\rule{0.250pt}{0.400pt}}
\multiput(717.00,649.58)(0.534,0.494){25}{\rule{0.529pt}{0.119pt}}
\multiput(717.00,648.17)(13.903,14.000){2}{\rule{0.264pt}{0.400pt}}
\multiput(732.00,663.58)(0.497,0.494){25}{\rule{0.500pt}{0.119pt}}
\multiput(732.00,662.17)(12.962,14.000){2}{\rule{0.250pt}{0.400pt}}
\multiput(746.00,677.58)(0.625,0.492){21}{\rule{0.600pt}{0.119pt}}
\multiput(746.00,676.17)(13.755,12.000){2}{\rule{0.300pt}{0.400pt}}
\multiput(761.00,689.58)(0.625,0.492){21}{\rule{0.600pt}{0.119pt}}
\multiput(761.00,688.17)(13.755,12.000){2}{\rule{0.300pt}{0.400pt}}
\multiput(776.00,701.58)(0.756,0.491){17}{\rule{0.700pt}{0.118pt}}
\multiput(776.00,700.17)(13.547,10.000){2}{\rule{0.350pt}{0.400pt}}
\multiput(791.00,711.58)(0.704,0.491){17}{\rule{0.660pt}{0.118pt}}
\multiput(791.00,710.17)(12.630,10.000){2}{\rule{0.330pt}{0.400pt}}
\multiput(805.00,721.59)(0.844,0.489){15}{\rule{0.767pt}{0.118pt}}
\multiput(805.00,720.17)(13.409,9.000){2}{\rule{0.383pt}{0.400pt}}
\multiput(820.00,730.59)(0.844,0.489){15}{\rule{0.767pt}{0.118pt}}
\multiput(820.00,729.17)(13.409,9.000){2}{\rule{0.383pt}{0.400pt}}
\multiput(835.00,739.59)(1.103,0.485){11}{\rule{0.957pt}{0.117pt}}
\multiput(835.00,738.17)(13.013,7.000){2}{\rule{0.479pt}{0.400pt}}
\multiput(850.00,746.59)(1.103,0.485){11}{\rule{0.957pt}{0.117pt}}
\multiput(850.00,745.17)(13.013,7.000){2}{\rule{0.479pt}{0.400pt}}
\multiput(865.00,753.59)(1.214,0.482){9}{\rule{1.033pt}{0.116pt}}
\multiput(865.00,752.17)(11.855,6.000){2}{\rule{0.517pt}{0.400pt}}
\multiput(879.00,759.59)(1.601,0.477){7}{\rule{1.300pt}{0.115pt}}
\multiput(879.00,758.17)(12.302,5.000){2}{\rule{0.650pt}{0.400pt}}
\multiput(894.00,764.59)(1.601,0.477){7}{\rule{1.300pt}{0.115pt}}
\multiput(894.00,763.17)(12.302,5.000){2}{\rule{0.650pt}{0.400pt}}
\multiput(909.00,769.60)(2.090,0.468){5}{\rule{1.600pt}{0.113pt}}
\multiput(909.00,768.17)(11.679,4.000){2}{\rule{0.800pt}{0.400pt}}
\multiput(924.00,773.60)(1.943,0.468){5}{\rule{1.500pt}{0.113pt}}
\multiput(924.00,772.17)(10.887,4.000){2}{\rule{0.750pt}{0.400pt}}
\multiput(938.00,777.61)(3.141,0.447){3}{\rule{2.100pt}{0.108pt}}
\multiput(938.00,776.17)(10.641,3.000){2}{\rule{1.050pt}{0.400pt}}
\multiput(953.00,780.61)(3.141,0.447){3}{\rule{2.100pt}{0.108pt}}
\multiput(953.00,779.17)(10.641,3.000){2}{\rule{1.050pt}{0.400pt}}
\put(968,783.17){\rule{3.100pt}{0.400pt}}
\multiput(968.00,782.17)(8.566,2.000){2}{\rule{1.550pt}{0.400pt}}
\put(983,784.67){\rule{3.373pt}{0.400pt}}
\multiput(983.00,784.17)(7.000,1.000){2}{\rule{1.686pt}{0.400pt}}
\put(997,785.67){\rule{3.614pt}{0.400pt}}
\multiput(997.00,785.17)(7.500,1.000){2}{\rule{1.807pt}{0.400pt}}
\put(1012,786.67){\rule{3.614pt}{0.400pt}}
\multiput(1012.00,786.17)(7.500,1.000){2}{\rule{1.807pt}{0.400pt}}
\put(1042,786.67){\rule{3.373pt}{0.400pt}}
\multiput(1042.00,787.17)(7.000,-1.000){2}{\rule{1.686pt}{0.400pt}}
\put(1027.0,788.0){\rule[-0.200pt]{3.613pt}{0.400pt}}
\put(1071,785.17){\rule{3.100pt}{0.400pt}}
\multiput(1071.00,786.17)(8.566,-2.000){2}{\rule{1.550pt}{0.400pt}}
\put(1086,783.67){\rule{3.614pt}{0.400pt}}
\multiput(1086.00,784.17)(7.500,-1.000){2}{\rule{1.807pt}{0.400pt}}
\put(1101,782.17){\rule{2.900pt}{0.400pt}}
\multiput(1101.00,783.17)(7.981,-2.000){2}{\rule{1.450pt}{0.400pt}}
\multiput(1115.00,780.95)(3.141,-0.447){3}{\rule{2.100pt}{0.108pt}}
\multiput(1115.00,781.17)(10.641,-3.000){2}{\rule{1.050pt}{0.400pt}}
\multiput(1130.00,777.95)(3.141,-0.447){3}{\rule{2.100pt}{0.108pt}}
\multiput(1130.00,778.17)(10.641,-3.000){2}{\rule{1.050pt}{0.400pt}}
\multiput(1145.00,774.95)(3.141,-0.447){3}{\rule{2.100pt}{0.108pt}}
\multiput(1145.00,775.17)(10.641,-3.000){2}{\rule{1.050pt}{0.400pt}}
\multiput(1160.00,771.95)(2.918,-0.447){3}{\rule{1.967pt}{0.108pt}}
\multiput(1160.00,772.17)(9.918,-3.000){2}{\rule{0.983pt}{0.400pt}}
\multiput(1174.00,768.94)(2.090,-0.468){5}{\rule{1.600pt}{0.113pt}}
\multiput(1174.00,769.17)(11.679,-4.000){2}{\rule{0.800pt}{0.400pt}}
\put(1189,764.67){\rule{0.723pt}{0.400pt}}
\multiput(1189.00,765.17)(1.500,-1.000){2}{\rule{0.361pt}{0.400pt}}
\put(1056.0,787.0){\rule[-0.200pt]{3.613pt}{0.400pt}}
\put(466.0,131.0){\rule[-0.200pt]{0.400pt}{175.616pt}}
\put(466.0,131.0){\rule[-0.200pt]{175.616pt}{0.400pt}}
\put(1195.0,131.0){\rule[-0.200pt]{0.400pt}{175.616pt}}
\put(466.0,860.0){\rule[-0.200pt]{175.616pt}{0.400pt}}
\end{picture}


==> NLiqNGas.tex <==
% GNUPLOT: LaTeX picture
\setlength{\unitlength}{0.240900pt}
\ifx\plotpoint\undefined\newsavebox{\plotpoint}\fi
\sbox{\plotpoint}{\rule[-0.200pt]{0.400pt}{0.400pt}}%
\begin{picture}(1500,900)(0,0)
\sbox{\plotpoint}{\rule[-0.200pt]{0.400pt}{0.400pt}}%
\put(466.0,131.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(446,131){\makebox(0,0)[r]{ 0}}
\put(1175.0,131.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(466.0,252.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(446,252){\makebox(0,0)[r]{ 0.2}}
\put(1175.0,252.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(466.0,374.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(446,374){\makebox(0,0)[r]{ 0.4}}
\put(1175.0,374.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(466.0,495.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(446,495){\makebox(0,0)[r]{ 0.6}}
\put(1175.0,495.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(466.0,617.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(446,617){\makebox(0,0)[r]{ 0.8}}
\put(1175.0,617.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(466.0,738.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(446,738){\makebox(0,0)[r]{ 1}}
\put(1175.0,738.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(466.0,860.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(446,860){\makebox(0,0)[r]{ 1.2}}
\put(1175.0,860.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(466.0,131.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(466,90){\makebox(0,0){ 0.2}}
\put(466.0,840.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(556.0,131.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(556,90){\makebox(0,0){ 0.3}}
\put(556.0,840.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(646.0,131.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(646,90){\makebox(0,0){ 0.4}}
\put(646.0,840.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(736.0,131.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(736,90){\makebox(0,0){ 0.5}}
\put(736.0,840.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(826.0,131.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(826,90){\makebox(0,0){ 0.6}}
\put(826.0,840.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(916.0,131.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(916,90){\makebox(0,0){ 0.7}}
\put(916.0,840.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(1006.0,131.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(1006,90){\makebox(0,0){ 0.8}}
\put(1006.0,840.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(1096.0,131.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(1096,90){\makebox(0,0){ 0.9}}
\put(1096.0,840.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(1186.0,131.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(1186,90){\makebox(0,0){ 1}}
\put(1186.0,840.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(466.0,131.0){\rule[-0.200pt]{0.400pt}{175.616pt}}
\put(466.0,131.0){\rule[-0.200pt]{175.616pt}{0.400pt}}
\put(1195.0,131.0){\rule[-0.200pt]{0.400pt}{175.616pt}}
\put(466.0,860.0){\rule[-0.200pt]{175.616pt}{0.400pt}}
\put(325,495){\makebox(0,0){n}}
\put(830,29){\makebox(0,0){T}}
\sbox{\plotpoint}{\rule[-0.500pt]{1.000pt}{1.000pt}}%
\sbox{\plotpoint}{\rule[-0.200pt]{0.400pt}{0.400pt}}%
\put(1035,820){\makebox(0,0)[r]{${n}_{liq}$}}
\sbox{\plotpoint}{\rule[-0.500pt]{1.000pt}{1.000pt}}%
\sbox{\plotpoint}{\rule[-0.200pt]{0.400pt}{0.400pt}}%
\put(1055.0,820.0){\rule[-0.200pt]{24.090pt}{0.400pt}}
\put(466,855){\usebox{\plotpoint}}
\multiput(466.00,853.92)(0.576,-0.493){23}{\rule{0.562pt}{0.119pt}}
\multiput(466.00,854.17)(13.834,-13.000){2}{\rule{0.281pt}{0.400pt}}
\multiput(481.00,840.92)(0.576,-0.493){23}{\rule{0.562pt}{0.119pt}}
\multiput(481.00,841.17)(13.834,-13.000){2}{\rule{0.281pt}{0.400pt}}
\multiput(496.00,827.92)(0.536,-0.493){23}{\rule{0.531pt}{0.119pt}}
\multiput(496.00,828.17)(12.898,-13.000){2}{\rule{0.265pt}{0.400pt}}
\multiput(510.00,814.92)(0.625,-0.492){21}{\rule{0.600pt}{0.119pt}}
\multiput(510.00,815.17)(13.755,-12.000){2}{\rule{0.300pt}{0.400pt}}
\multiput(525.00,802.92)(0.684,-0.492){19}{\rule{0.645pt}{0.118pt}}
\multiput(525.00,803.17)(13.660,-11.000){2}{\rule{0.323pt}{0.400pt}}
\multiput(540.00,791.92)(0.684,-0.492){19}{\rule{0.645pt}{0.118pt}}
\multiput(540.00,792.17)(13.660,-11.000){2}{\rule{0.323pt}{0.400pt}}
\multiput(555.00,780.92)(0.637,-0.492){19}{\rule{0.609pt}{0.118pt}}
\multiput(555.00,781.17)(12.736,-11.000){2}{\rule{0.305pt}{0.400pt}}
\multiput(569.00,769.92)(0.684,-0.492){19}{\rule{0.645pt}{0.118pt}}
\multiput(569.00,770.17)(13.660,-11.000){2}{\rule{0.323pt}{0.400pt}}
\multiput(584.00,758.92)(0.684,-0.492){19}{\rule{0.645pt}{0.118pt}}
\multiput(584.00,759.17)(13.660,-11.000){2}{\rule{0.323pt}{0.400pt}}
\multiput(599.00,747.92)(0.756,-0.491){17}{\rule{0.700pt}{0.118pt}}
\multiput(599.00,748.17)(13.547,-10.000){2}{\rule{0.350pt}{0.400pt}}
\multiput(614.00,737.92)(0.704,-0.491){17}{\rule{0.660pt}{0.118pt}}
\multiput(614.00,738.17)(12.630,-10.000){2}{\rule{0.330pt}{0.400pt}}
\multiput(628.00,727.92)(0.756,-0.491){17}{\rule{0.700pt}{0.118pt}}
\multiput(628.00,728.17)(13.547,-10.000){2}{\rule{0.350pt}{0.400pt}}
\multiput(643.00,717.92)(0.756,-0.491){17}{\rule{0.700pt}{0.118pt}}
\multiput(643.00,718.17)(13.547,-10.000){2}{\rule{0.350pt}{0.400pt}}
\multiput(658.00,707.93)(0.844,-0.489){15}{\rule{0.767pt}{0.118pt}}
\multiput(658.00,708.17)(13.409,-9.000){2}{\rule{0.383pt}{0.400pt}}
\multiput(673.00,698.92)(0.704,-0.491){17}{\rule{0.660pt}{0.118pt}}
\multiput(673.00,699.17)(12.630,-10.000){2}{\rule{0.330pt}{0.400pt}}
\multiput(687.00,688.93)(0.844,-0.489){15}{\rule{0.767pt}{0.118pt}}
\multiput(687.00,689.17)(13.409,-9.000){2}{\rule{0.383pt}{0.400pt}}
\multiput(702.00,679.92)(0.756,-0.491){17}{\rule{0.700pt}{0.118pt}}
\multiput(702.00,680.17)(13.547,-10.000){2}{\rule{0.350pt}{0.400pt}}
\multiput(717.00,669.93)(0.844,-0.489){15}{\rule{0.767pt}{0.118pt}}
\multiput(717.00,670.17)(13.409,-9.000){2}{\rule{0.383pt}{0.400pt}}
\multiput(732.00,660.93)(0.786,-0.489){15}{\rule{0.722pt}{0.118pt}}
\multiput(732.00,661.17)(12.501,-9.000){2}{\rule{0.361pt}{0.400pt}}
\multiput(746.00,651.93)(0.844,-0.489){15}{\rule{0.767pt}{0.118pt}}
\multiput(746.00,652.17)(13.409,-9.000){2}{\rule{0.383pt}{0.400pt}}
\multiput(761.00,642.93)(0.844,-0.489){15}{\rule{0.767pt}{0.118pt}}
\multiput(761.00,643.17)(13.409,-9.000){2}{\rule{0.383pt}{0.400pt}}
\multiput(776.00,633.93)(0.844,-0.489){15}{\rule{0.767pt}{0.118pt}}
\multiput(776.00,634.17)(13.409,-9.000){2}{\rule{0.383pt}{0.400pt}}
\multiput(791.00,624.93)(0.786,-0.489){15}{\rule{0.722pt}{0.118pt}}
\multiput(791.00,625.17)(12.501,-9.000){2}{\rule{0.361pt}{0.400pt}}
\multiput(805.00,615.93)(0.844,-0.489){15}{\rule{0.767pt}{0.118pt}}
\multiput(805.00,616.17)(13.409,-9.000){2}{\rule{0.383pt}{0.400pt}}
\multiput(820.00,606.93)(0.844,-0.489){15}{\rule{0.767pt}{0.118pt}}
\multiput(820.00,607.17)(13.409,-9.000){2}{\rule{0.383pt}{0.400pt}}
\multiput(835.00,597.93)(0.844,-0.489){15}{\rule{0.767pt}{0.118pt}}
\multiput(835.00,598.17)(13.409,-9.000){2}{\rule{0.383pt}{0.400pt}}
\multiput(850.00,588.93)(0.844,-0.489){15}{\rule{0.767pt}{0.118pt}}
\multiput(850.00,589.17)(13.409,-9.000){2}{\rule{0.383pt}{0.400pt}}
\multiput(865.00,579.93)(0.786,-0.489){15}{\rule{0.722pt}{0.118pt}}
\multiput(865.00,580.17)(12.501,-9.000){2}{\rule{0.361pt}{0.400pt}}
\multiput(879.00,570.93)(0.844,-0.489){15}{\rule{0.767pt}{0.118pt}}
\multiput(879.00,571.17)(13.409,-9.000){2}{\rule{0.383pt}{0.400pt}}
\multiput(894.00,561.92)(0.756,-0.491){17}{\rule{0.700pt}{0.118pt}}
\multiput(894.00,562.17)(13.547,-10.000){2}{\rule{0.350pt}{0.400pt}}
\multiput(909.00,551.93)(0.844,-0.489){15}{\rule{0.767pt}{0.118pt}}
\multiput(909.00,552.17)(13.409,-9.000){2}{\rule{0.383pt}{0.400pt}}
\multiput(924.00,542.93)(0.786,-0.489){15}{\rule{0.722pt}{0.118pt}}
\multiput(924.00,543.17)(12.501,-9.000){2}{\rule{0.361pt}{0.400pt}}
\multiput(938.00,533.92)(0.756,-0.491){17}{\rule{0.700pt}{0.118pt}}
\multiput(938.00,534.17)(13.547,-10.000){2}{\rule{0.350pt}{0.400pt}}
\multiput(953.00,523.93)(0.844,-0.489){15}{\rule{0.767pt}{0.118pt}}
\multiput(953.00,524.17)(13.409,-9.000){2}{\rule{0.383pt}{0.400pt}}
\multiput(968.00,514.92)(0.756,-0.491){17}{\rule{0.700pt}{0.118pt}}
\multiput(968.00,515.17)(13.547,-10.000){2}{\rule{0.350pt}{0.400pt}}
\multiput(983.00,504.92)(0.704,-0.491){17}{\rule{0.660pt}{0.118pt}}
\multiput(983.00,505.17)(12.630,-10.000){2}{\rule{0.330pt}{0.400pt}}
\multiput(997.00,494.92)(0.756,-0.491){17}{\rule{0.700pt}{0.118pt}}
\multiput(997.00,495.17)(13.547,-10.000){2}{\rule{0.350pt}{0.400pt}}
\multiput(1012.00,484.92)(0.756,-0.491){17}{\rule{0.700pt}{0.118pt}}
\multiput(1012.00,485.17)(13.547,-10.000){2}{\rule{0.350pt}{0.400pt}}
\multiput(1027.00,474.92)(0.684,-0.492){19}{\rule{0.645pt}{0.118pt}}
\multiput(1027.00,475.17)(13.660,-11.000){2}{\rule{0.323pt}{0.400pt}}
\multiput(1042.00,463.92)(0.704,-0.491){17}{\rule{0.660pt}{0.118pt}}
\multiput(1042.00,464.17)(12.630,-10.000){2}{\rule{0.330pt}{0.400pt}}
\multiput(1056.00,453.92)(0.625,-0.492){21}{\rule{0.600pt}{0.119pt}}
\multiput(1056.00,454.17)(13.755,-12.000){2}{\rule{0.300pt}{0.400pt}}
\multiput(1071.00,441.92)(0.625,-0.492){21}{\rule{0.600pt}{0.119pt}}
\multiput(1071.00,442.17)(13.755,-12.000){2}{\rule{0.300pt}{0.400pt}}
\multiput(1086.00,429.92)(0.625,-0.492){21}{\rule{0.600pt}{0.119pt}}
\multiput(1086.00,430.17)(13.755,-12.000){2}{\rule{0.300pt}{0.400pt}}
\multiput(1101.00,417.92)(0.536,-0.493){23}{\rule{0.531pt}{0.119pt}}
\multiput(1101.00,418.17)(12.898,-13.000){2}{\rule{0.265pt}{0.400pt}}
\multiput(1115.00,404.92)(0.534,-0.494){25}{\rule{0.529pt}{0.119pt}}
\multiput(1115.00,405.17)(13.903,-14.000){2}{\rule{0.264pt}{0.400pt}}
\multiput(1130.58,389.81)(0.494,-0.531){27}{\rule{0.119pt}{0.527pt}}
\multiput(1129.17,390.91)(15.000,-14.907){2}{\rule{0.400pt}{0.263pt}}
\multiput(1145.58,373.70)(0.494,-0.566){27}{\rule{0.119pt}{0.553pt}}
\multiput(1144.17,374.85)(15.000,-15.852){2}{\rule{0.400pt}{0.277pt}}
\multiput(1160.58,355.98)(0.494,-0.791){25}{\rule{0.119pt}{0.729pt}}
\multiput(1159.17,357.49)(14.000,-20.488){2}{\rule{0.400pt}{0.364pt}}
\multiput(1174.58,332.71)(0.494,-1.181){27}{\rule{0.119pt}{1.033pt}}
\multiput(1173.17,334.86)(15.000,-32.855){2}{\rule{0.400pt}{0.517pt}}
\multiput(1189.61,290.52)(0.447,-4.258){3}{\rule{0.108pt}{2.767pt}}
\multiput(1188.17,296.26)(3.000,-14.258){2}{\rule{0.400pt}{1.383pt}}
\put(1035,779){\makebox(0,0)[r]{${n}_{gas}$}}
\put(1055.0,779.0){\rule[-0.200pt]{24.090pt}{0.400pt}}
\put(466,131){\usebox{\plotpoint}}
\put(717,130.67){\rule{3.614pt}{0.400pt}}
\multiput(717.00,130.17)(7.500,1.000){2}{\rule{1.807pt}{0.400pt}}
\put(466.0,131.0){\rule[-0.200pt]{60.466pt}{0.400pt}}
\put(761,131.67){\rule{3.614pt}{0.400pt}}
\multiput(761.00,131.17)(7.500,1.000){2}{\rule{1.807pt}{0.400pt}}
\put(732.0,132.0){\rule[-0.200pt]{6.986pt}{0.400pt}}
\put(805,132.67){\rule{3.614pt}{0.400pt}}
\multiput(805.00,132.17)(7.500,1.000){2}{\rule{1.807pt}{0.400pt}}
\put(820,133.67){\rule{3.614pt}{0.400pt}}
\multiput(820.00,133.17)(7.500,1.000){2}{\rule{1.807pt}{0.400pt}}
\put(835,134.67){\rule{3.614pt}{0.400pt}}
\multiput(835.00,134.17)(7.500,1.000){2}{\rule{1.807pt}{0.400pt}}
\put(850,135.67){\rule{3.614pt}{0.400pt}}
\multiput(850.00,135.17)(7.500,1.000){2}{\rule{1.807pt}{0.400pt}}
\put(865,136.67){\rule{3.373pt}{0.400pt}}
\multiput(865.00,136.17)(7.000,1.000){2}{\rule{1.686pt}{0.400pt}}
\put(879,137.67){\rule{3.614pt}{0.400pt}}
\multiput(879.00,137.17)(7.500,1.000){2}{\rule{1.807pt}{0.400pt}}
\put(894,139.17){\rule{3.100pt}{0.400pt}}
\multiput(894.00,138.17)(8.566,2.000){2}{\rule{1.550pt}{0.400pt}}
\put(909,140.67){\rule{3.614pt}{0.400pt}}
\multiput(909.00,140.17)(7.500,1.000){2}{\rule{1.807pt}{0.400pt}}
\put(924,142.17){\rule{2.900pt}{0.400pt}}
\multiput(924.00,141.17)(7.981,2.000){2}{\rule{1.450pt}{0.400pt}}
\put(938,144.17){\rule{3.100pt}{0.400pt}}
\multiput(938.00,143.17)(8.566,2.000){2}{\rule{1.550pt}{0.400pt}}
\put(953,146.17){\rule{3.100pt}{0.400pt}}
\multiput(953.00,145.17)(8.566,2.000){2}{\rule{1.550pt}{0.400pt}}
\multiput(968.00,148.61)(3.141,0.447){3}{\rule{2.100pt}{0.108pt}}
\multiput(968.00,147.17)(10.641,3.000){2}{\rule{1.050pt}{0.400pt}}
\multiput(983.00,151.61)(2.918,0.447){3}{\rule{1.967pt}{0.108pt}}
\multiput(983.00,150.17)(9.918,3.000){2}{\rule{0.983pt}{0.400pt}}
\multiput(997.00,154.61)(3.141,0.447){3}{\rule{2.100pt}{0.108pt}}
\multiput(997.00,153.17)(10.641,3.000){2}{\rule{1.050pt}{0.400pt}}
\multiput(1012.00,157.61)(3.141,0.447){3}{\rule{2.100pt}{0.108pt}}
\multiput(1012.00,156.17)(10.641,3.000){2}{\rule{1.050pt}{0.400pt}}
\multiput(1027.00,160.60)(2.090,0.468){5}{\rule{1.600pt}{0.113pt}}
\multiput(1027.00,159.17)(11.679,4.000){2}{\rule{0.800pt}{0.400pt}}
\multiput(1042.00,164.60)(1.943,0.468){5}{\rule{1.500pt}{0.113pt}}
\multiput(1042.00,163.17)(10.887,4.000){2}{\rule{0.750pt}{0.400pt}}
\multiput(1056.00,168.60)(2.090,0.468){5}{\rule{1.600pt}{0.113pt}}
\multiput(1056.00,167.17)(11.679,4.000){2}{\rule{0.800pt}{0.400pt}}
\multiput(1071.00,172.59)(1.304,0.482){9}{\rule{1.100pt}{0.116pt}}
\multiput(1071.00,171.17)(12.717,6.000){2}{\rule{0.550pt}{0.400pt}}
\multiput(1086.00,178.59)(1.304,0.482){9}{\rule{1.100pt}{0.116pt}}
\multiput(1086.00,177.17)(12.717,6.000){2}{\rule{0.550pt}{0.400pt}}
\multiput(1101.00,184.59)(1.214,0.482){9}{\rule{1.033pt}{0.116pt}}
\multiput(1101.00,183.17)(11.855,6.000){2}{\rule{0.517pt}{0.400pt}}
\multiput(1115.00,190.59)(0.956,0.488){13}{\rule{0.850pt}{0.117pt}}
\multiput(1115.00,189.17)(13.236,8.000){2}{\rule{0.425pt}{0.400pt}}
\multiput(1130.00,198.59)(0.844,0.489){15}{\rule{0.767pt}{0.118pt}}
\multiput(1130.00,197.17)(13.409,9.000){2}{\rule{0.383pt}{0.400pt}}
\multiput(1145.00,207.58)(0.625,0.492){21}{\rule{0.600pt}{0.119pt}}
\multiput(1145.00,206.17)(13.755,12.000){2}{\rule{0.300pt}{0.400pt}}
\multiput(1160.58,219.00)(0.494,0.570){25}{\rule{0.119pt}{0.557pt}}
\multiput(1159.17,219.00)(14.000,14.844){2}{\rule{0.400pt}{0.279pt}}
\multiput(1174.58,235.00)(0.494,0.976){27}{\rule{0.119pt}{0.873pt}}
\multiput(1173.17,235.00)(15.000,27.187){2}{\rule{0.400pt}{0.437pt}}
\multiput(1189.61,264.00)(0.447,3.811){3}{\rule{0.108pt}{2.500pt}}
\multiput(1188.17,264.00)(3.000,12.811){2}{\rule{0.400pt}{1.250pt}}
\put(776.0,133.0){\rule[-0.200pt]{6.986pt}{0.400pt}}
\put(466.0,131.0){\rule[-0.200pt]{0.400pt}{175.616pt}}
\put(466.0,131.0){\rule[-0.200pt]{175.616pt}{0.400pt}}
\put(1195.0,131.0){\rule[-0.200pt]{0.400pt}{175.616pt}}
\put(466.0,860.0){\rule[-0.200pt]{175.616pt}{0.400pt}}
\end{picture}

